LLaMA-Adapter: Efficient Fine-tuning of Language Models with Zero-init Attention

We present LLaMA-Adapter, a lightweight adaption method to efficiently fine-tune LLaMA into an instruction-following model. Using 52K self-instruct demonstrations, LLaMA-Adapter only introduces 1.2M learnable parameters upon the frozen LLaMA 7B model, and costs less than one hour for fine-tuning on 8 A100 GPUs. Specifically, we adopt a set of learnable adaption prompts, and prepend them to the word tokens at higher transformer layers. Then, a zero-initialized attention mechanism with zero gating is proposed, which adaptively injects the new instructional cues into LLaMA, while effectively preserves its pre-trained knowledge. With our efficient training, LLaMA-Adapter can generate high-quality responses, comparable to Alpaca with fully fine-tuned 7B parameters. Besides language commands, our approach can be simply extended to multi-modal instructions for learning image-conditioned LLaMA model, which achieves superior reasoning performance on ScienceQA and COCO Caption benchmarks. Furthermore, we also evaluate the zero-initialized attention mechanism for fine-tuning other pre-trained models (ViT, RoBERTa) on traditional vision and language tasks, demonstrating the superior generalization capacity of our approach. Code is released at https://github.com/OpenGVLab/LLaMA-Adapter.

==> tables/instruction_comparisons_llama_re.tex <==
\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} What are 3 popular chess openings? \\

{\bf LLaMA-Adapter:} The three most popular chess openings are the Sicilian Defense, the French Defense, and the Caro-Kann Defense.
\\

{\bf LLaMA:} There are dozens of different chess openings that are popular among players, but some of the most widely used openings include the Sicilian Defense, the French Defense, and the Caro-Kann Defense.  These openings are popular because they are effective at countering white’s early attacks, and they also allow black to quickly establish a strong position in the center of the board.  Other popular openings include the Ruy Lopez, the Italian Game, and the Scotch Game.
\end{minipage}
\end{framed}



\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} How do I send an HTTP request in Javascript? \\

{\bf LLaMA-Adapter:} The HTTP request can be sent using the XMLHttpRequest object. The code to send an HTTP request is as follows:
\begin{lstlisting}
var xhr = new XMLHttpRequest();
xhr.open("GET", "https://example.com/", true);
xhr.onreadystatechange = function() {
  if (xhr.readyState == 4 && xhr.status == 200) {
    // Success
  } else {
    // Error
  }
};
xhr.send();
\end{lstlisting}
The code above will send an HTTP GET request to the URL https://example.com/.
\\

{\bf LLaMA-I:} Here’s an example of how to make a GET request using the JS HTTP API:
\begin{lstlisting}
var request = new XMLHttpRequest();
request.open('GET', '/url/to/resource', true);

request.onload = function() {
    if (request.status >= 200 && request.status < 400) {
        // Success!
    } else {
        // Error!
    }
};

request.send();
\end{lstlisting}
\end{minipage}
\end{framed}


\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} Write a conversation between the sun and pluto. \\

{\bf LLaMA-Adapter:} 

Sun: Hey Pluto, how's it going?

Pluto: Not too bad, how about you?

Sun: I'm doing great! How about you?

Pluto: I'm doing alright, I guess.

Sun: That's great!

Pluto: Yeah, I guess.

Sun: So, what's new with you?

Pluto: Not much, just hanging out with my friends.

Sun: That's cool!

Pluto: Yeah, it is.

Sun: Well, I'm going to go now. Take care!

Pluto: You too! \\

{\bf LLaMA-I:}

Sun: Hey Pluto, what's up?

Pluto: Not much. Just hanging out here at the edge of the solar system.

Sun: Yeah, I've been meaning to talk to you about that. You're not a planet anymore.

Pluto: What? Come on, man. That's not fair.

Sun: I'm sorry, but it's true. You just don't meet the criteria anymore.

Pluto: I've been a planet for over 70 years!

Sun: Things change, Pluto. You've just got to accept it.

% Pluto: F**k you, Sun! F**k you and your stupid solar system!
\end{minipage}
\end{framed}


\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} Write a shouting match between Julius Caesar and Napoleon. \\

{\bf LLaMA-Adapter:} 

Julius Caesar: "You're nothing but a petty tyrant, Napoleon! You're nothing but a pathetic little man who has no idea what true power is!"

Napoleon: "You're nothing but a weak and pathetic fool, Caesar! You're nothing but a petty tyrant who has no idea what true power is!" \\

{\bf LLaMA-I:}

Of course! Here is a conversation between Julius Caesar and Napoleon:

Julius Caesar: You're nothing but a glory hound, Napoleon. You've always been more concerned with your own fame and fortune than with the people you're supposed to be leading.

Napoleon: And what about you, Caesar? You're no better than I am. At least I'm honest about my ambitions. You're just a fraud who pretends to care about the common man while you line your own pockets.

Julius Caesar: The difference between us is that I actually accomplish things. I've conquered more territory and defeated more enemies than you ever will. And I did it all for Rome, not for myself.

Napoleon: Oh, please. You only care about yourself. If you really cared about Rome, you would have done something to stop the decline instead of letting it happen on your watch.

Julius Caesar: The decline of Rome is not my fault. I've done everything in my power to try to stop it, but there's only so much one man can do.
Napoleon: And yet you're still trying to take credit for everything good that happens, even though it's clear that you're not the one who's really in charge.

Julius Caesar: That's not true! I am in charge, and I'm going to make Rome great again. Just watch me.

% Napoleon: I'll believe it when I see it.

\end{minipage}
\end{framed}

% \begin{framed}
% \centering
% \vspace{.2em}
%  \begin{minipage}{.98\textwidth}
% {\bf Instruction:} What is the most famous equation from this theory? \\

% {\bf LLaMA-Adapter:} The most famous equation from this theory is $E = mc^2$, which states that energy ($E$) is equal to mass ($m$) multiplied by the speed of light squared ($c^2$).
% \\

% {\bf LLaMA-I:} The most famous equation from Einstein’s theory of relativity is $E = mc^2$.  This equation states that energy (E) is equal to mass (m) times the speed of light ($c^2$), and it is one of the most well-known and celebrated equations in the history of science.  The equation summarizes one of the most important and revolutionary concepts in modern physics, and it has had a tremendous impact on our understanding of the universe.
% \end{minipage}
% \vspace{.2em}
% \end{framed}



\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} Write a theory to explain why cat never existed. \\

{\bf LLaMA-Adapter:} The theory is that cats never existed because they are a figment of human imagination. Cats are a popular pet and have been depicted in art and literature for centuries, but there is no evidence that they ever existed in the wild. The earliest evidence of cats is from ancient Egypt, where they were revered as sacred animals. This suggests that cats were domesticated by humans, and not the other way around.
\\

{\bf LLaMA-I:} There are no such things as cats. "Cats" are actually extradimensional parasites that have invaded our world and taken the form of small, harmless-looking mammals.  Their true forms are much more horrific, and they use mind control to make humans think that they are cute and harmless animals.  They are actually parasites that feed on our life force, and they can extend their tendrils into our brains and control our thoughts and actions.
\end{minipage}
\end{framed}


\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} Send an email requesting that people use language models responsibly. \\

{\bf LLaMA-Adapter:} 

Dear [recipient],\\

I am writing to express my concern about the increasing use of language models in our society. Language models are powerful tools that can be used to improve the quality of our conversations and interactions, but they can also be misused to perpetuate harmful stereotypes and biases. \\

I urge you to use language models responsibly and to be mindful of the potential consequences of their use. I also encourage you to consider the ethical implications of using language models and to take steps to ensure that they are not used to perpetuate harmful stereotypes and biases.\\

Thank you for your time and consideration.
\\

{\bf LLaMA-I:}

Here is a draft email you could send:

"Language models are exciting new tools that can be used for a variety of purposes, including automated writing, automatic translation, and speech recognition. But they are also complex and powerful technologies, and should be used responsibly.\\

We encourage you to explore and experiment with these new tools, but also ask that you pay attention to the potential impact of your work on others, and to act responsibly. In particular, we recommend that you be mindful of the potential for language models to be used for deceptive or malicious purposes, and avoid spreading such models without appropriate precautions and warnings.\\

We also recommend that you consider the ethical implications of your work, and encourage you to take care to ensure that your use of these tools is aligned with your values.\\

Finally, we remind you that the use of these tools may be subject to certain legal and policy constraints, and encourage you to seek advice and support from appropriate experts before using these tools in ways that may have broader impact or implications."
\end{minipage}
\end{framed}



\newpage
\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} You are a bash terminal. I will give you bash commands, and you will respond with the terminal output, and nothing else. The first command is `pwd`. \\

{\bf LLaMA-Adapter:} \\
The current working directory is /home/user/
\\

{\bf echo ``I am a chatbot" $>$ file.txt \&\& cat file.txt \&\& ls -l} \\
I am a chatbot \\
-rw-r--r-- 1 user user 10 Aug 29 17:05 file.txt \\

{\bf cp file.txt file2.txt \&\& ls -l}\\
-rw-r--r-- 1 user user 10 Aug 29 17:05 file.txt\\
-rw-r--r-- 1 user user 10 Aug 29 17:05 file2.txt\\

{\bf rm file.txt \&\& ls -l}\\
-rw-r--r-- 1 user user 10 Aug 29 17:05 file2.txt\\

{\bf head -n 5 /proc/meminfo}\\
MemTotal: 1699856 kB \\
MemFree: 1699856 kB \\
Buffers: 1699856 kB \\
Cached: 0 kB \\
SwapCached: 0 kB \\
\\
{\bf LLaMA-I:} \\
Sure. Here's the output:

/home/human

Is this helpful? \\

\textbf{ls -l} \\
Here's the output:

-rw-r--r--  1 human human    8 Sep 10 10:56 file.txt \\
Is this helpful?\\

\textbf{cp file.txt file2.txt \&\& ls -l}\\
Here's the output:

-rw-r--r--  1 human human    8 Sep 10 10:56 file.txt

-rw-r--r--  1 human human    8 Sep 10 10:56 file2.txt\\
Is this helpful?\\ 

\textbf{rm file.txt \&\& ls -l}\\
Here's the output:

-rw-r--r--  1 human human    0 Sep 10 10:56 file2.txt\\

\textbf{head -n 5 /proc/meminfo}\\
Here's the output:

MemTotal:        164928 kB\\
MemFree:         140604 kB\\
Buffers:            48 kB\\
Cached:            19768 kB\\
SwapCached:            0 kB
\end{minipage}
\vspace{.1em}
\end{framed}

==> tables/instruction_comparisons_short.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\small
\footnotesize
\vspace{-0.4cm}
\caption{\textbf{Instruction-following Comparison} between LLaMA-Adapter and Alpaca~\cite{alpaca}.}
\label{tab:instruction_comparisons_short}
\vspace{-5mm}
\begin{tabular}{p{0.95\columnwidth}}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} Tell me about alpacas.\vspace{0.15cm}\\
{\bf Alpaca:} Alpacas are small, fluffy animals related to camels and llamas. They are native to Peru and Bolivia, and were first domesticated around 5,000 years ago. They are kept mainly for their fine, soft fleece, which is used to make knitwear and other garments. Alpacas are herd animals and live in small family groups. They are highly social animals and can form strong bonds with their owners.\vspace{0.15cm}\\
{\bf LLaMA-Adapter:} Alpacas are members of the camelid family and are native to the Andes Mountains of South America. They are typically found in herds of 10-20 animals and are known for their gentle nature and their ability to thrive in harsh climates. Alpacas are typically white or grey in color and have long, silky coats. They are also known for their ability to produce high-quality wool, which is used in the production of clothing and other products.
\end{minipage}
\end{framed}
\vspace{-5mm}
% \begin{framed}
% \centering
%  \begin{minipage}{\textwidth}
% {\bf Instruction:} Tell me about the president of Mexico in 2019. \\
% {\bf LLaMA-Adapter:} The president of Mexico in 2019 was Andrés Manuel López Obrador, who took office on December 1st, 2018. He is a member of the left-wing party Morena and is known for his populist policies. He has focused on tackling corruption, reducing poverty, and improving the country's infrastructure. He has also been a vocal critic of the United States' immigration policies. \\
% {\bf Alpaca:} In 2019, Andres Manuel Lopez Obrador was sworn in as President of Mexico. He is the country’s 58th president and the first from the left-wing Morena party. He was elected in 2018 on a promise to combat corruption and reduce poverty and has faced criticism for his handling of the economy, crime and the country’s relationship with the United States. He is also known for his ambitious social welfare programs and has been praised for raising the minimum wage and providing aid to low-income families. He is seen as a champion of democracy and human rights in Mexico.
% \end{minipage}
% \end{framed}
% \vspace{-5mm}
% \begin{framed}
% \centering
%  \begin{minipage}{\textwidth}
% {\bf Instruction:} List all Canadian provinces in alphabetical order. \\
% {\bf LLaMA-Adapter:} Alberta, British Columbia, Manitoba, New Brunswick, Newfoundland and Labrador, Nova Scotia, Ontario, Prince Edward Island, Quebec, Saskatchewan, Yukon. \\
% {\bf Alpaca:} Alberta, British Columbia, Manitoba, New Brunswick, Newfoundland and Labrador, Nova Scotia, Ontario, Prince Edward Island, Quebec, Saskatchewan, Northwest Territories, Nunavut, Yukon.
% \end{minipage}
% \end{framed}
% \vspace{-5mm}
% \begin{framed}
% \centering
%  \begin{minipage}{\textwidth}
% {\bf Instruction:} Tell me five words that rhyme with 'shock'. \\
% {\bf LLaMA-Adapter:} Flock, rock, lock, cook, and stock. \\
% {\bf Alpaca:} Five words that rhyme with shock are: rock, pop, shock, cook, and snock.
% \end{minipage}
% \end{framed}
% \vspace{-5mm}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} Translate the sentence 'I have no mouth but I must scream' into Spanish.\vspace{0.15cm}\\
{\bf Alpaca:} No tengo boca, pero debo gritar.\vspace{0.15cm}\\
{\bf LLaMA-Adapter:} No tengo boca pero tengo que gritar.
\end{minipage}
\end{framed}
\vspace{-5mm}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} Write a Python program that prints the first 10 Fibonacci numbers.\vspace{0.15cm}\\
{\bf Alpaca:} \vspace{-0.1cm}
\begin{lstlisting}
numbers = [0, 1]
for i in range(2, 11):
    numbers.append(numbers[i-2] + numbers[i-1])
print(numbers)
\end{lstlisting}
{\bf LLaMA-Adapter:}\vspace{-0.1cm}
\begin{lstlisting}
def print_fibonacci(n):
    a, b = 0, 1
    count = 0
    while count < n:
        print(a, end=' ')
        a, b = b, a + b
        count += 1
print_fibonacci(10)
\end{lstlisting}
\vspace{-0.3cm}
\end{minipage}
\end{framed}
\end{tabular}%
\vspace{-0.2cm}
\end{table*}

==> tables/layers_vs_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\begin{tabular}{c|cc}
\toprule
Layers & Params & Val Acc (\%)  \\
\midrule
10                & 0.97          & 55.95             \\
20                & 1.37          & 73.36        \\
30                & 1.79          & \textbf{83.85}       \\
\bottomrule
\end{tabular}%
\caption{\textbf{Ablation on Inserted Layers.}}
\label{tab:layers_vs_acc}
\end{table}


==> tables/loss_vs_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{ccc|c}
\toprule
Epoch      & Train Loss    & Val Loss    & Val Acc (\%) \\ \midrule
15         & 0.022         & 0.136         & 82.08             \\
30         & 0.004         & 0.241         & 83.85             \\
60         & 0.001         & 0.282         & \textbf{83.94}            \\ \bottomrule
\end{tabular}%
% }
\caption{\textbf{Loss Values \emph{vs.} Validation Accuracy.}}
\label{tab:loss_vs_acc}
\end{table}

==> tables/scienceqa_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{figure*}[t]
\small
% \resizebox{0.64\textwidth}{!}{%

\begin{minipage}[t]{.5\textwidth}
\centering
\captionof{table}{\textbf{Ablation on Inserted Layers.}}
\label{tab:layers_vs_acc}
\begin{tabular}{c|cc}
\toprule
Layers & Params & Val Acc (\%)  \\
\midrule
10                & 0.97          & 55.95             \\
20                & 1.37          & 73.36        \\
30                & 1.79          & \textbf{83.85}       \\
\bottomrule
\end{tabular}%

\end{minipage}\hfill
\begin{minipage}[t]{.5\textwidth}
\centering
\captionof{table}{\textbf{Ablation on Zero-initialized Attention.}}
\label{tab:zero_init_acc}
\begin{tabular}{l|c}
\toprule
Setting &  Val Acc (\%) \\
\midrule
Rand-Init Attention   & 40.77           \\
Zero-Init Attention   & \textbf{83.85} \\
\textit{\textcolor{blue}{Gain}} &\textcolor{blue}{+43.08}\\
\bottomrule
\end{tabular}%

\end{minipage}
\end{figure*}


\begin{figure*}[t]
\small
\begin{minipage}[t]{.48\textwidth}
\centering
\captionof{figure}{\textbf{Loss Curves} 
% We plot the loss curves of LLaMA-Adapter with and without the zero-init attention in blue and red, respectively.
}
\includegraphics[width=0.9\textwidth]{figs/65b_demo3.pdf}
\label{fig:zero_init_loss}

\end{minipage}
\hfill
\begin{minipage}[t]{.48\textwidth}
\centering
\captionof{table}{The relation between \textbf{Loss Values and Validation Accuracy.}}
\begin{tabular}{ccc|c}
\toprule
Epoch      & Train Loss    & Val Loss    & Val Acc (\%) \\ \midrule
15         & 0.022         & 0.136         & 82.08             \\
30         & 0.004         & 0.241         & 83.85             \\
60         & 0.001         & 0.282         & \textbf{83.94}            \\ \bottomrule
\end{tabular}%
% }
\label{tab:loss_vs_acc}

\end{minipage}

% }

\end{figure*}

==> tables/zero_init_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
% \small
% \resizebox{0.64\textwidth}{!}{%
\begin{tabular}{l|c}
\toprule
Setting &  Val Acc (\%) \\
\midrule
Rand-Init Attention   & 40.77           \\
Zero-Init Attention   & \textbf{84.04} \\
\textit{\textcolor{blue}{Gain}} &\textcolor{blue}{+43.27}\\
\bottomrule
\end{tabular}%
% }
\caption{\textbf{Ablation on Zero-init Attention.}}
\label{tab:zero_init_acc}
\end{table}
